Testing Permanent Oracles -- Revisited

Suppose we are given an oracle that claims to approximate the permanent for most matrices X, where X is chosen from the Gaussian ensemble (the matrix entries are i.i.d. univariate complex Gaussians). Can we test that the oracle satisfies this claim? This paper gives a polynomial-time algorithm for the task. The oracle-testing problem is of interest because a recent paper of Aaronson and Arkhipov showed that if there is a polynomial-time algorithm for simulating boson-boson interactions in quantum mechanics, then an approximation oracle for the permanent (of the type described above) exists in BPP^NP. Since computing the permanent of even 0/1 matrices is #P-complete, this seems to demonstrate more computational power in quantum mechanics than Shor's factoring algorithm does. However, unlike factoring, which is in NP, it was unclear previously how to test the correctness of an approximation oracle for the permanent, and this is the contribution of the paper. The technical difficulty overcome here is that univariate polynomial self-correction, which underlies similar oracle-testing algorithms for permanent over finite fields --- and whose discovery led to a revolution in complexity theory --- does not seem to generalize to complex (or even, real) numbers. We believe that this tester will motivate further progress on understanding the permanent of Gaussian matrices.

==> matrix.tex <==
Here we will desribe a test that looks at all the $2k$ subspaces
orginating from a given matrix $X$ and tests that the function is in
fact close to being linear (in the sense desribed in the above
section) in every one of those subspaces.

The guarantee, is again two fold: $(1)$ if the function is in fact
close to the permanent on a large fraction of the inputs, the test
accepts with probability $1-\frac{1}{\poly(n)}$; $(2)$ if the function
does not satisfy ``$\ell_2$-norm guarantee'' for a large fraction of
the inputs, then the test fails with probability at least $1-\exp(n)$
over the coin tosses of the test.
%  the test
% passes, then with good probability over the coin tosses, I will learn
% to write this shit in a better way.

\paragraph{Tester.}
The test consists of two parts, first is the \emph{linearity} test and
the second is a \emph{range} test. The \emph{linearity} test involves repeating
the following $n^a$ times: 

\vspace{4mm}
\emph{
Sample a matrix $X.$ Let
$g_1,\ldots,g_k$ be the entries in the first row of $X.$ Let
$X_i$ be the minor obtained by removing the first row and the
$i^{\textrm{th}}$ column from $X.$ Test the following,
\[ \left(f_k(X) - \sum_{i=1}^k g_i f_{k-1}(X_i)\right)^2 \le
\delta^2\cdot k!\]
Output \texttt{Reject} if it does not hold.
}
\vspace{4mm}

\noindent The \emph{range} test involves repeating the following $T^4/n^b$
times:

\vspace{4mm}
\emph{Sample a $(k-1)\times (k-1)$ matrix $X.$ Test that $f_{k-1}(X)^2
  \le \frac{T^2}{4}(k-1)!.$ Output \texttt{Reject} if it does not hold.
}
\vspace{4mm}


\paragraph{Analysis.}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "reals"
%%% End: 


==> optim-symbs.tex <==
%%% Symbols for optimization, inapprox. related results %%%

% common operators
\newcommand{\sdp}{{\sf SDP}}
\newcommand{\qp}{\mathrm{qp}}
\newcommand{\opt}{{\sf opt}}
\newcommand{\val}{{\sf val}}
\newcommand{\round}{{\sf round}}
\newcommand{\Round}{{\sf ROUND}}
\newcommand{\minimize}{\text{minimize}}
\newcommand{\maximize}{\text{maximize}}
\newcommand{\subjectto}{\text{subject to}}
\newcommand{\lp}{\mathsf{lp}}

% Ideally should be in ugc-hardness
\newcommand{\Inf}{\mathrm{Inf}}
\newcommand{\Dict}{{\sc Dict}}

% convex hull
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\simplex}{{\sf Sim}}

%%% %%%


==> prettyrefs.tex <==
%%% Pretty Ref Macros %%%

\usepackage{prettyref}

\newrefformat{eq}{\textup{(\ref{#1})}}
\newrefformat{lem}{Lemma~\ref{#1}}
\newrefformat{thm}{Theorem~\ref{#1}}
\newrefformat{cha}{Chapter~\ref{#1}}
\newrefformat{sec}{Section~\ref{#1}}
\newrefformat{tab}{Table~\ref{#1} on page~\pageref{#1}}
\newrefformat{fig}{Figure~\ref{#1} on page~\pageref{#1}}
\newrefformat{def}{Definition~\ref{#1}}


%%% %%%


==> technical.tex <==
{\color{red} Sushant: I am just writing the technical claims
  here. There are a lot of parameters here, but I think the technical
  core of the proof is complete. I just wanted to complete the chain
  of technical claims.}

Here we will desribe a test that looks at all the $2k$ subspaces
orginating from a given matrix $X$ and tests that the function is in
fact close to being linear (in the sense desribed in the above
section) in every one of those subspaces.

The guarantee, is again two fold: $(1)$ if the function is in fact
close to the permanent on a large fraction of the inputs, the test
accepts with probability $1-\frac{1}{\poly(n)}$; $(2)$ if the function
does not satisfy ``$\ell_2$-norm guarantee'' for a large fraction of
the inputs, then the test fails with probability at least $1-\exp(n)$
over the coin tosses of the test.
%  the test
% passes, then with good probability over the coin tosses, I will learn
% to write this shit in a better way.

\paragraph{Tester.}


\vspace{4mm}



\paragraph{Analysis.}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "reals"
%%% End: 



